Assessing Security and Performances of Consensus algorithms for Permissioned Blockchains

Blockchain is a novel technology that is rising a lot of interest in the industrial and re- search sectors because its properties of decentralisation, immutability and data integrity. Initially, the underlying consensus mechanism has been designed for permissionless block- chain on trustless network model through the proof-of-work, i.e. a mathematical challenge which requires high computational power. This solution suffers of poor performances, hence alternative consensus algorithms as the proof-of-stake have been proposed. Conversely, for permissioned blockchain, where participants are known and authenti- cated, variants of distributed consensus algorithms have been employed. However, most of them comes out without formal expression of security analysis and trust assumptions because the absence of an established knowledge. Therefore the lack of adequate analysis on these algorithms hinders any cautious evaluation of their effectiveness in a real-world setting where systems are deployed over trustless networks, i.e. Internet ...

==> chapters_s/cap_04_benchmark/04_01_pascal-related.tex <==
% !TEX root = ../Tesi-1side.tex

\section{Related Works} \label{s:pascal-related}



==> chapters_s/cap_05_conclusion/12_future.tex <==
% !TEX root = ../../Tesi-1side.tex

The main objective to carry on the work of this thesis is the integration of the two parts. The idea is to define an \textit{elastic dependable framework} which allows to reconfigure runtime the system in a decentralised manner.%, thus by relying on a permissioned blockchain as underlying infrastructure.

\begin{figure}[!htb]
	\centering
	\includegraphics[scale=0.05]{figures/conclusion/elastic_framework}
	\itcaption{Decentralised Elastic Dependable Framework}
	\label{fig:elastic-dependable-framework}
\end{figure}

Figure \ref{fig:elastic-dependable-framework} shows a possible architecture of the elastic dependable framework. Ideally, it is deployed on top of a permissioned blockchain, used as underlying infrastructure, anchored with a permissionless blockchain as proposed for the 2LBC architecture. Compared to PASCAL, events triggering reconfigurations are not only workload changes, yet also faults and attacks, thus further modules beyond PASCAL are necessary. Specifically, a \textit{fault/attack detector}\footnote{Along this directions, my contributions are NiTREC \cite{baldoni2014towards} and NIRVANA \cite{ciccotelli2015nirvana}, two failure detection/prediction systems which correlate observed metrics to infer whether the system is behaving correctly or there is a fault}, by revealing (or forecasting) a tough conditions such as a fault or an attack, can interact with the controller to properly reconfigure the system.

Therefore, the membership of the permissioned network might be managed runtime through voting smart contracts. Therefore, subverted nodes which behave maliciously can be voted out (as we assessed with Proof-of-Authority algorithms in Chapter \ref{c10:poa}) to maintain a honest membership.

\smallskip
This framework, so, will be a decentralised extension of PASCAL in which decisions of reconfigurations are taken with the consensus of network members.
For this scope, one of the main challenges moves along consensus protocols for permissioned blockchain. Indeed, solutions based on PBFT fails in performances and scalability, yet solution based on Proof-of-Authority seems to be too weak in consistency as they propose \textit{eventual consensus} which can be not ideal for scenarios where forks may lead to huge harm. Therefore, in order to speed up the system while guaranteeing \textit{safety} and \textit{liveness} with Byzantine faults, will be investigated new protocols specific for permissioned blockchain.

\smallskip
For what concern instead the permissionless blockchain (anchored as second layer), being Proof-of-Work so heavy and cost ineffective, I plan to investigate some different model to encourage users to behave honestly. Currently, cryptocurrencies-based blockchain like Bitcoin and Ethereum employ monetary rewards for users who mine correctly blocks. 
Sociology community has widely proven as without an incentive, ethic will lose \cite{hardin2009tragedy}. I propose so to replace the concept of \textit{incentive} with the concept of \textit{necessity}. Thereby, there can be found crucial factors which miners need to "survive"; thus, game theory can be exploited to define a game in which a player is discouraged to behave maliciously rather than encouraged to behave honestly.

%
%Thus, instead of giving a monetary reward to miners as incentive, can be exploited Models based on game theory can be investigated to study.

%for transaction log, whereas system reconfiguration are executed through smart contracts in order to involve all member of the network.
%

%The main idea is to employ the 2LBC architecture, thus a permissioned blockchain in the first layer anchored to a permissionless blockchain for the second layer.
%
%The membership of the first layer network might be managed runtime through voting smart contracts, as we assessed in Chapter \ref{c10:poa}.
%

 






 



\begin{comment}
Another important aspect we want to investigate is the economics behind this elastic model. What is the best model to price the elastic replication system? Who are the customers for this kind of service? The answers to these questions depend on the definition of a precise cost model that
can help to identify the market sectors where such replication mechanism could
be beneficial.

Finally, we are investigating how to make the MYSE architecture completely non-intrusive. i.e., so that the MYSE module does not need any information provided by the replicated service, such as the service times. This would enable and ease its employment in a wider range of applications.

Indeed, overall system performance does not scale adding new nodes, as the used total consensus algorithm has lower performance with additional nodes. In this section we propose the solutions to cope with them.

\smallskip
\noindent
\emph{Availability.} To mitigate such limitations, we propose a Byzantine Fault Tolerant solution based on PBFT~\cite{castro1999practical}. To tolerate up to $f$ Byzantine miners it requires $3f+1$ miners to provide both \textit{safety} and \textit{liveness}. This leads to higher availability level as honest miners need to wait just $f+1$ valid signatures to commit a txn. We can so tolerate up to $f$ \textit{silent} miners at the cost of weaker integrity guarantees; indeed data corruption is possible with just $f+1$ compromised miners, rather than all $N$ when total consensus is used. Anyway, the integrity of txns already witnessed in the second layer is still ensured thanks to the PoW.


\smallskip
\noindent
\emph{Scalability.} To improve scalability, we propose a \textit{data sharding} solution for permissioned (federated) blockchain, similar to \cite{luu2016secure} for permissionless blockchain. Specifically, we introduce a DHT-based ledger in which each miner, on the base of a \emph{keyspace partitioning}, only handles txns for specific subsets of keys. This approach permits tuning txn loads on miners and, consequently, makes the system more scalable. Furthermore, each key range has a configurable replication factor to enable fault tolerance. In our solution, contrarily to common DHT implementations, the miners involved in a \texttt{set} operation must achieve consensus before writing the operation in the local replica (hence in the local keyspace) of the redo log. This permits achieving strong consistency, hence avoiding consistency issues which mar well known DHT-based NoSQL databases, such as DynamoDB (\url{aws.amazon.com/dynamodb/}) and Cassandra (\url{wiki.apache.org/cassandra/}). Clearly, this comes at the cost of performance penalties, whose quantification depends on the technology and is beyond our scope here.

\begin{figure}[tb]
	\begin{center}
		\includegraphics[width=9.0cm]{figures/2lbc/dht} 
	\end{center}
	\itcaption{Example of the DHT-based ledger solution to achieve total replication in the FaaS scenario. The federation is composed by $M=3$ members (each one marked with a proper color), each one exposing $N=2$ miners (identified by a proper letter). Miners are disposed on the ring so as each member has all keys of the database sharded between its miners. The single miners keep only a subset proportional to the replication factor. In the example, the replication factor is $M=3$ and each miner maintains only $1/N=1/2$ of database keys.}
	\label{fig:dht}
\end{figure}

The solution to the FaaS scenario can e.g.\ change as follow: let \emph{M} be the number of federation members, each providing \emph{N} (rather than a single) miners. The DHT ring includes $M \cdot N$ nodes, the replication factor is set to \emph{M}, and miners can be placed over the ring so that the miners of each federation member collectively manage all the keys. Figure~\ref{fig:dht} shows an example of a FaaS federation composed by $M=3$ members, each exposing $N=2$ miners.

\end{comment}

==> ing-thesis/Acknowledgement.tex <==
\vspace{7cm} \hspace{7cm} \emph{A pippo}

